The Warm Gas in the MW: A Kinematical Model

We develop a kinematical model for the Milky Way Si IV-bearing gas to determine its density distribution and kinematics. This model is constrained by a column density line shape sample extracted from the {\it HST}/COS archival data, which contains 186 AGN sight lines. We find that the Si IV ion density distribution is dominated by an extended disk along the $z$-direction (above or below the midplane), i.e., $n(z)=n_0\exp(-(z/z_0)^{0.82})$, where $z_0$ is the scale height of $6.3_{-1.5}^{+1.6}$ kpc (northern hemisphere) and $3.6_{-0.9}^{+1.0}$ kpc (southern hemisphere). The density distribution of the disk in the radial direction shows a sharp edge at $15-20$ kpc given by, $n(r_{\rm XY})=n_0\exp(-(r_{\rm XY}/r_0)^{3.36})$, where $r_0 \approx 12.5\pm0.6$ kpc. The difference of density distributions over $r_{\rm XY}$ and $z$ directions indicates that the warm gas traced by \ion{Si}{4} is mainly associated with disk processes (e.g., feedback or cycling gas) rather than accretion. We estimate the mass of the warm gas (within 50 kpc) is $\log (M(50 {\rm kpc})/M_\odot)\approx8.1$ (assuming $Z\approx0.5Z_\odot$), and a $3\sigma$ upper limit of $\log (M(250 {\rm kpc})/M_\odot)\approx9.1$ (excluding the Magellanic system). Kinematically, the warm gas disk is nearly co-rotating with the stellar disk at $v_{\rm rot}=215\pm3\rm~km~s^{-1}$, which lags the midplane rotation by about $8\rm~km~s^{-1}~kpc^{-1}$ (within 5 kpc). Meanwhile, we note that the warm gas in the northern hemisphere has significant accretion with $v_{\rm acc}$ of $69\pm 7\rm ~km~s^{-1}$ at 10 kpc (an accretion rate of $-0.60_{-0.13}^{+0.11}~M_\odot\rm~yr^{-1}$), while in the southern hemisphere, there is no measurable accretion, with an upper limit of $0.4~M_\odot\rm~yr^{-1}$.

==> table_sample.tex <==
\tablehead{\colhead{Sightline} & \colhead{$l$} & \colhead{$b$ } & \colhead{$S/N$} & \colhead{$S/N$} & \colhead{$v_{\rm min}$} & \colhead{$v_{\rm max}$} & \colhead{$\log N$} & \colhead{$\sigma_{\log N}$} & \colhead{$v_{\rm c}$} & \colhead{$\sigma_{v_{\rm c}}$}\\
& deg. & deg. & Strong & Weak & $\kms$ & $\kms$ & dex & dex & $\kms$ & $\kms$ }
        Mrk 1392 & $   2.8$ & $  50.3$ & $ 24$ & $ 23$ & $-150$ & $  50$ & $13.75$ & $0.02$ & $ -37.1$ & $  1.2$ \\
LQAC 209+017 004 & $   2.9$ & $  71.8$ & $ 25$ & $ 25$ & $-140$ & $  30$ & $13.70$ & $0.01$ & $ -42.8$ & $  1.4$ \\
     PG 1352+183 & $   4.4$ & $  72.9$ & $ 37$ & $ 39$ & $-180$ & $  60$ & $13.65$ & $0.01$ & $ -45.0$ & $  1.1$ \\
        RBS 1768 & $   4.5$ & $ -48.5$ & $ 20$ & $ 20$ & $-220$ & $ -60$ & $13.17$ & $0.03$ & $-141.7$ & $  3.4$ \\
                 &          &          &       &       & $ -60$ & $ 120$ & $13.58$ & $0.02$ & $  29.7$ & $  1.6$ \\
LQAC 350-034 001 & $   5.5$ & $ -69.4$ & $ 17$ & $ 18$ & $-130$ & $ -70$ & $12.68$ & $0.07$ & $-102.2$ & $  2.6$ \\
                 &          &          &       &       & $ -70$ & $  50$ & $13.23$ & $0.03$ & $ -15.7$ & $  2.3$

